Single and Parallel Machine Scheduling with Variable Release Dates

In this paper we study a simple extension of the total weighted flowtime minimization problem for single and identical parallel machines. While the standard problem simply defines a set of jobs with their processing times and weights and assumes that all jobs have release date 0 and have no deadline, we assume that the release date of each job is a decision variable that is only constrained by a single global latest arrival deadline. To our knowledge, this simple yet practically highly relevant extension has never been studied. Our main contribution is that we show the NP- completeness of the problem even for the single machine case and provide an exhaustive empirical study of different typical approaches including genetic algorithms, tree search, and constraint programming.

==> npcompletenessproof-multiplemachines.tex <==
\subsubsection{The Parallel-Machine Problem is NP-Complete}

\begin{theorem}
    \probMulti is NP-complete. 
\end{theorem}
\begin{proof}
    \emph{NP membership.}
    Trivial, because guessing a solution is possible in polynomial time, and checking such a solution only requires linear time by evaluating $\phi$ for a number of $m$ times.
    
    \emph{NP-hardness.}
    Consider the weighted flowtime minimization problem for two machines \probUnconstrained as defined in \cite{lenstra1977complexity}; the $I$ qualifies the problem to be a parallel shop (here with two machines).
    Theorem 3b of the same paper shows this problem to be NP-hard.
    The following simple reduction shows that \probUnconstrained is a special case of \probMulti:
    Given an instance of \probUnconstrained, retain the specifications of $J$, $w_i$, $d_i$, and $m = 2$, and set $L = 0$.
    Clearly, all arrival times are then 0 and $\phi$ collapses to $\sum w_i C_i$, where we adopt the notation $C_i$ of completion times for job $i$.
    This identity directly proves the NP-hardness for the case $m = 2$.
    For cases $m > 2$, we can adopt the same reduction of {\sc Partition} conducted in \cite{lenstra1977complexity}.
    Clearly, if the number of machines increases, one can still check whether a decomposition of a set of integers into two sets with equal sums exist (the other machines but the first two will simply not be used).
    
    
\end{proof}

==> results/d0.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
    size &    naive &     mcts &  ga-random &    ga-rr &    ga-ff &  ga-rr-ff &    cplex &       cp &      ils \\
\midrule
  20 x 1 &    0.03\% &    1.56\% &      0.00\% &    0.00\% &    0.00\% &     0.00\% &    0.34\% &    0.37\% &    0.00\% \\
  30 x 1 &    0.01\% &    1.47\% &      0.00\% &    0.00\% &    0.01\% &     0.01\% &    0.49\% &    4.66\% &    0.00\% \\
  40 x 1 &    0.01\% &    1.48\% &      0.41\% &    0.00\% &    0.00\% &     0.00\% &    1.56\% &    0.00\% &    0.00\% \\
  60 x 1 &    0.01\% &    3.96\% &      0.01\% &    0.01\% &    0.00\% &     0.00\% &   15.92\% &    6.33\% &    6.33\% \\
  80 x 1 &    0.00\% &    3.01\% &      0.73\% &    0.00\% &    0.06\% &     5.60\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 100 x 1 &    0.00\% &    5.26\% &      2.67\% &    5.35\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 120 x 1 &    0.00\% &    7.20\% &      5.59\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 140 x 1 &    0.00\% &    8.10\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 160 x 1 &    0.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 180 x 1 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 200 x 1 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 300 x 1 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 400 x 1 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 500 x 1 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% &    0.00\% \\
  20 x 2 &    0.32\% &    5.38\% &      0.06\% &    0.05\% &    0.04\% &     0.05\% &    0.46\% &    0.04\% &    0.00\% \\
  30 x 2 &    0.06\% &    7.05\% &      0.10\% &    0.11\% &    0.10\% &     0.05\% &    1.28\% &    0.03\% &    0.00\% \\
  40 x 2 &    0.04\% &    7.29\% &      0.21\% &    0.07\% &    0.02\% &     0.04\% &    0.41\% &    0.00\% &    0.00\% \\
  60 x 2 &    0.17\% &    5.61\% &      0.43\% &    0.12\% &    0.05\% &     0.05\% &    1.94\% &    0.04\% &    0.00\% \\
  80 x 2 &    0.15\% &    6.06\% &      1.80\% &    0.26\% &    0.02\% &     0.02\% &    6.53\% &    0.04\% &    0.00\% \\
 100 x 2 &    1.93\% &    6.70\% &      0.56\% &    0.00\% &    3.82\% &     3.82\% &   14.75\% &   11.48\% &    8.15\% \\
 120 x 2 &    1.52\% &    5.99\% &      0.00\% &    1.51\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 140 x 2 & 1000.00\% &    0.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% & 1000.00\% \\
 160 x 2 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 180 x 2 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 200 x 2 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 300 x 2 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 400 x 2 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 500 x 2 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% &    0.00\% \\
  20 x 3 &    0.59\% &    9.91\% &      0.12\% &    0.20\% &    0.17\% &     0.26\% &    0.60\% &    0.34\% &    0.00\% \\
  30 x 3 &    0.89\% &    9.33\% &      0.25\% &    0.00\% &    0.13\% &     0.08\% &    0.86\% &    0.24\% &    0.02\% \\
  40 x 3 &    0.18\% &    8.20\% &      0.13\% &    0.30\% &    0.03\% &     0.08\% &    0.59\% &    0.14\% &    0.00\% \\
  60 x 3 &    0.38\% &    8.81\% &      0.83\% &    0.10\% &    0.00\% &     0.00\% &    2.51\% &    0.06\% &    0.00\% \\
  80 x 3 &    0.00\% &    9.53\% &      1.02\% &    1.30\% &    1.07\% &     1.08\% &    7.20\% &    1.23\% &    1.01\% \\
 100 x 3 &    0.44\% &    7.70\% &      1.89\% &    0.20\% &    0.03\% &     0.03\% &    4.89\% &    0.31\% &    0.00\% \\
 120 x 3 &    0.00\% &    4.85\% &      0.80\% &    0.17\% &    0.01\% &     0.01\% & 1000.00\% &    0.25\% & 1000.00\% \\
 140 x 3 & 1000.00\% & 1000.00\% &      7.48\% &    6.62\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% &    0.00\% \\
 160 x 3 & 1000.00\% &    0.00\% &   1000.00\% & 1000.00\% & 1000.00\% &     0.00\% & 1000.00\% & 1000.00\% &   20.00\% \\
 180 x 3 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 200 x 3 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 300 x 3 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 400 x 3 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% &  200.00\% &    0.00\% \\
 500 x 3 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% &    0.00\% \\
  20 x 5 &    0.83\% &   16.91\% &      0.01\% &    0.36\% &    0.34\% &     0.43\% &    0.40\% &    0.92\% &    0.00\% \\
  30 x 5 &    1.03\% &   12.07\% &      0.46\% &    0.00\% &    0.05\% &     0.07\% &    0.70\% &    0.77\% &    0.03\% \\
  40 x 5 &    1.16\% &   17.83\% &      0.87\% &    0.00\% &    0.10\% &     0.10\% &    0.86\% &    0.43\% &    0.18\% \\
  60 x 5 &    1.25\% &   11.82\% &      0.80\% &    0.40\% &    0.02\% &     0.00\% &    2.99\% &    0.82\% &    0.06\% \\
  80 x 5 &    4.52\% &   14.01\% &      3.90\% &    3.50\% &    3.15\% &     4.38\% &    7.76\% &    3.81\% &    0.00\% \\
 100 x 5 &    1.44\% &   11.30\% &      0.68\% &    0.62\% &    0.31\% &     0.27\% &    8.16\% &    1.13\% &    0.00\% \\
 120 x 5 &    4.40\% &   14.72\% &      3.70\% &    3.17\% &    2.97\% &     2.98\% &    9.46\% &    3.92\% &    0.00\% \\
 140 x 5 &    8.58\% &   18.95\% &      6.37\% &    6.81\% &    2.96\% &     5.44\% &   12.22\% &    5.08\% &    0.00\% \\
 160 x 5 &    4.38\% &   17.37\% &      3.72\% &    2.14\% &    0.87\% &     1.49\% &   35.34\% &    0.00\% &    1.93\% \\
 180 x 5 &    8.43\% &   15.42\% &      2.91\% &    0.08\% &    0.00\% &     2.48\% &   54.59\% &    3.98\% &    4.73\% \\
 200 x 5 &    0.00\% & 1000.00\% &      3.24\% & 1000.00\% &    1.21\% &     2.58\% &  105.03\% & 1000.00\% & 1000.00\% \\
 300 x 5 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% &    0.00\% & 1000.00\% &  100.00\% \\
 400 x 5 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% & 1000.00\% &    0.00\% \\
 500 x 5 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% &    0.00\% &      NaN &      NaN \\
  20 x 9 &    1.58\% &   33.18\% &      0.28\% &    0.05\% &    0.23\% &     0.48\% &    0.00\% &    0.21\% &    0.19\% \\
  30 x 9 &    3.11\% &   33.24\% &      0.18\% &    0.38\% &    0.00\% &     0.00\% &    0.22\% &    0.71\% &    0.13\% \\
  40 x 9 &    1.96\% &   31.93\% &      2.35\% &    0.66\% &    0.00\% &     0.05\% &    0.84\% &    1.75\% &    0.37\% \\
  60 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
  80 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 100 x 9 &   23.25\% &   19.45\% &      2.86\% &    3.42\% &    3.03\% &     1.32\% &    6.81\% &    3.99\% &    0.00\% \\
 120 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 140 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 160 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 180 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 200 x 9 &      NaN &      NaN &        NaN &      NaN &      NaN &       NaN &      NaN &      NaN &      NaN \\
 300 x 9 & 1000.00\% & 1000.00\% &   1000.00\% & 1000.00\% & 1000.00\% &  1000.00\% & 1000.00\% &    0.00\% &      NaN \\
 400 x 9 & 1000.00\% & 1000.00\% &   1000.00\% &    0.00\% & 1000.00\% &  1000.00\% & 1000.00\% &      NaN &      NaN \\
 500 x 9 &    0.22\% & 1000.00\% &      2.82\% &    0.00\% &    0.09\% &     0.09\% &      NaN &      NaN &      NaN \\
\bottomrule
\end{tabular}

==> results/d1.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
   size &  naive &   mcts &  ga-random &  ga-rr &  ga-ff &  ga-rr-ff &  cplex &    cp &   ils \\
\midrule
 20 x 1 &  0.16\% &  0.33\% &      0.00\% &  0.00\% &  0.00\% &     0.00\% &  0.41\% & 0.00\% & 0.00\% \\
 30 x 1 &  0.18\% &  1.23\% &      0.54\% &  0.00\% &  0.00\% &     0.00\% &  2.14\% & 0.00\% & 0.00\% \\
 40 x 1 &  0.16\% &  2.98\% &      0.79\% &  0.03\% &  0.00\% &     0.03\% &  9.08\% & 2.29\% & 0.00\% \\
 60 x 1 &  0.08\% &  6.17\% &      0.61\% &  0.06\% &  0.07\% &     0.07\% & 14.74\% &  $\infty$ & 0.00\% \\
 20 x 2 &  0.99\% &  7.82\% &      0.16\% &  0.18\% &  0.17\% &     0.17\% &  0.62\% & 0.00\% & 0.00\% \\
 30 x 2 &  0.59\% & 11.25\% &      1.08\% &  0.45\% &  0.37\% &     0.40\% &  3.23\% & 0.00\% & 0.00\% \\
 40 x 2 &  0.51\% & 12.68\% &      1.24\% &  0.61\% &  0.50\% &     0.40\% &  5.15\% & 0.05\% & 0.00\% \\
 60 x 2 &  0.24\% & 17.71\% &      1.60\% &  0.47\% &  0.26\% &     0.29\% & 11.03\% &  $\infty$ & 0.00\% \\
\bottomrule
\end{tabular}



==> results/d3_max.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
    size &  naive &   mcts &  ga-random &  ga-rr &  ga-ff &  ga-rr-ff &   cplex &    cp &   ils \\
\midrule
  20 x 1 &  1.99\% &  5.50\% &      4.17\% &  1.99\% &  1.22\% &     1.99\% &  14.90\% & 1.20\% & 0.23\% \\
  30 x 1 &  1.91\% &  9.88\% &     11.47\% &  1.91\% &  1.91\% &     1.91\% &  34.85\% &  $\infty$ & 0.32\% \\
  40 x 1 &  1.02\% & 17.71\% &     21.59\% &  1.02\% &  1.02\% &     1.02\% & 100.00\% &  $\infty$ & 0.12\% \\
  60 x 1 &  0.48\% & 17.55\% &     29.68\% &  0.48\% &  0.48\% &     0.48\% &  82.93\% &  $\infty$ & 0.11\% \\
  80 x 1 &  0.22\% & 18.59\% &     36.46\% &  0.22\% &  0.22\% &     0.13\% &  84.13\% &  $\infty$ & 0.04\% \\
 100 x 1 &  0.14\% & 17.74\% &     29.42\% &  0.14\% &  0.12\% &     0.12\% & 100.00\% &  $\infty$ & 0.00\% \\
  20 x 2 &  7.09\% & 19.99\% &      7.00\% &  3.10\% &  2.47\% &     3.06\% &   2.62\% & 1.18\% & 0.99\% \\
  30 x 2 &  5.28\% & 28.04\% &     10.28\% &  4.87\% &  3.06\% &     3.06\% &  26.89\% & 2.01\% & 0.95\% \\
  40 x 2 &  2.51\% & 28.87\% &     19.20\% &  3.46\% &  1.75\% &     1.68\% &  27.92\% &  $\infty$ & 0.82\% \\
  60 x 2 &  4.08\% & 43.21\% &     41.39\% &  2.88\% &  0.82\% &     0.82\% &  40.40\% &  $\infty$ & 0.59\% \\
  80 x 2 &  0.90\% & 28.77\% &     15.69\% &  1.66\% &  0.50\% &     0.45\% &  56.48\% &  $\infty$ & 0.12\% \\
 100 x 2 &  0.55\% & 45.18\% &     28.13\% &  2.27\% &  0.39\% &     0.36\% &  53.28\% &  $\infty$ & 0.02\% \\
  20 x 3 & 12.45\% & 21.48\% &      5.41\% &  4.76\% &  3.97\% &     3.44\% &   2.19\% & 1.44\% & 1.53\% \\
  30 x 3 &  8.36\% & 32.90\% &     23.49\% &  8.25\% &  2.94\% &     2.71\% &   7.45\% & 1.31\% & 1.37\% \\
  40 x 3 &  2.84\% & 26.37\% &     15.34\% &  7.02\% &  2.31\% &     2.55\% &  15.53\% & 1.21\% & 1.29\% \\
  60 x 3 &  4.33\% & 32.58\% &     17.48\% &  4.59\% &  1.24\% &     1.29\% &  37.45\% &  $\infty$ & 0.86\% \\
  80 x 3 &  0.97\% & 29.77\% &     21.30\% &  3.61\% &  0.80\% &     0.65\% &  36.93\% &  $\infty$ & 0.25\% \\
 100 x 3 &  0.97\% & 37.55\% &     19.10\% &  4.26\% &  0.54\% &     0.54\% &  52.55\% &  $\infty$ & 0.05\% \\
  20 x 5 &  4.84\% & 18.60\% &      0.64\% &  1.56\% &  1.07\% &     3.57\% &   0.55\% & 1.66\% & 1.20\% \\
  30 x 5 &  3.01\% & 19.13\% &      4.83\% &  4.21\% &  3.11\% &     2.89\% &   2.17\% & 1.63\% & 0.14\% \\
  40 x 5 &  4.79\% & 21.13\% &      8.16\% &  5.94\% &  1.99\% &     3.11\% &   4.48\% & 2.02\% & 0.40\% \\
  60 x 5 &  3.75\% & 25.12\% &     31.65\% &  4.46\% &  1.28\% &     1.28\% &  14.00\% & 2.11\% & 0.36\% \\
  80 x 5 &  2.16\% & 27.92\% &     10.76\% &  3.82\% &  1.09\% &     1.63\% &  33.25\% &  $\infty$ & 0.21\% \\
 100 x 5 &  4.47\% & 32.69\% &     32.49\% &  4.37\% &  0.89\% &     1.06\% &  33.10\% &  $\infty$ & 0.39\% \\
\bottomrule
\end{tabular}



==> theoreticalresults.tex <==

\begin{lemma}
    \label{theorem:giantjobaslateaspossible}
    A schedule $\pi$ for an instance of \probOne with $p_i,w_i \geq 1$ for all jobs $i\in J$ and containing a giant job $g$ is sub-optimal if there is a job $j$ scheduled after $g$ but that could be started before $g$ and still finish not later than the deadline $d$.
\end{lemma}

\begin{proof}
    By Lemma \ref{theorem:giantjobnotlaterthandeadline} we can assume that $\pi$ starts $g$ not later than the deadline $d$, and since $j$ can be placed before $g$ and finish still before $d$, in fact $\pi$ must start $g$ even strictly earlier than $d$.
    
    Now consider the schedule $\pi'$ in which job $j$ is moved to directly precede $g$.
    Since its finishing time is still prior to $d$, also the giant job $g$ will still start not later than $d$ under $\pi'$.
    Furthermore observe that
    \begin{align*}
        \phi(\pi) & = \sum\limits_{i\in I} w_ip_i + w_gp_g + w_j(p_g -d + p_j   + \smashoperator{\sum\limits_{i: \pi(i) < \pi(j), i\neq g}}p_i) +  M\\
        \phi(\pi') & = \sum\limits_{i\in I} w_ip_i + w_jp_j + w_gp_g + \smashoperator{\sum\limits_{\substack{i \in J_{-g}\setminus I\\ \pi(i) < \pi(j)}}}w_ip_j + M,
    \end{align*}
    where $M$ contains the contributions of all the jobs started later than $j$ by $\pi$ (and hence $\pi'$).
    Taking the difference, we obtain
    \begin{align*}
        \phi(\pi') - \phi(\pi) & = w_jp_j + w_gp_g + \smashoperator{\sum\limits_{\substack{i \in J_{-g}\setminus I:\\ \pi(i) < \pi(j)}}}w_ip_j - (w_gp_g + w_j(p_g -d + p_j   + \smashoperator{\sum\limits_{\substack{i: \pi(i) < \pi(j),\\ i\neq g}}}p_i))\\
        & = \smashoperator{\sum\limits_{\substack{i \in J_{-g}\setminus I:\\ \pi(i) < \pi(j)}}}w_ip_j - \smashoperator{\sum\limits_{\substack{i: \pi(i) < \pi(j),\\ i\neq g}}}w_jp_i + dw_j - p_gw_j\\
        & < \sum\limits_{\substack{i,j \in J_{-g},\\i\neq j}}w_ip_j + dw_j - p_gw_j\\
        &  < 2 \smashoperator{\sum\limits_{\substack{i,j \in J_{-g}}}}w_ip_j - p_gw_j < 0,
    \end{align*}
    where the last inequality follows from the lower bound on the weight $p_g$ of the giant job in property (1) of Def. \ref{def:giant} and the fact that $w_j \geq 1$.
\end{proof}
